Improving the transferability of speech separation by meta-learning

Speech separation aims to separate multiple speech sources from a speech mixture. Although speech separation is well-solved on some existing English speech separation benchmarks, it is worthy of more investigation on the generalizability of speech separation models on the accents or languages unseen during training. This paper adopts meta-learning based methods to improve the transferability of speech separation models. With the meta-learning based methods, we discovered that only using speech data with one accent, the native English accent, as our training data, the models still can be adapted to new unseen accents on the Speech Accent Archive. We compared the results with a human-rated native-likeness of accents, showing that the transferability of MAML methods has less relation to the similarity of data between the training and testing phase compared to the typical transfer learning methods. Furthermore, we found that models can deal with different language data from the CommonVoice corpus during the testing phase. Most of all, the MAML methods outperform typical transfer learning methods when it comes to new accents, new speakers, new languages, and noisy environments.

==> tables/English_accents_3spk_noise.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{4pt}
\begin{tabular}{cccccccccccccc}
\toprule
model & method & f.t. & Al  & Ga & Ha & It & Ku & Li & Me & Ru & Ta & Th  & overall \\
\midrule
conv  & joint  & - & 4.73	& 7.63	& 2.35	& 6.02	& 5.63	& 2.92	& 5.03	& 5.74	& 7.55	& 7.11	& 5.38\\
conv  & joint  & \checkmark & 4.72	& 7.23	& 2.48	& 6.14	& 5.15	& 2.82	& 5.48	& 5.56	& 7.09	& 7.17	& 5.28\\
dprnn & joint  & - & 5.43	& 8.52	& 3.78	& 7.46	& 6.46	& 4.71	& 7.10	& 6.96	& 8.54	& 8.88	& 6.61\\
dprnn & joint  & \checkmark  & 5.61	& 8.48	& 3.62	& 7.42	& 6.76	& 4.84	& 8.61	& 6.86	& 8.58	& 8.99	& 6.66\\
\midrule
conv  & fomaml & \checkmark & 5.90	& 7.81	& 3.79	& 7.09	& 6.44	& 4.75	& 3.65	& 6.66	& 7.46	& 7.60	& 6.31\\
conv  & maml   & \checkmark & 6.95	& 10.3	& 4.70 & 9.22 & 7.67	& 6.98 & 11.08 & 8.8 & 10.34 & 9.87 & 8.08\\
dprnn & fomaml & \checkmark & 7.31	& 8.86	& 5.13	& 8.59	& 8.05	& 6.17	& 9.16	& 7.87	& 8.90	& 9.01	& 7.71 \\
\bottomrule
\end{tabular}
\caption{Results of joint training and MAML methods under the 3-speaker setting on the 10 target accents of the Speech Accent Archive with Musan noise added.}
\label{tab:accent_result_2spk}
\end{table*}

==> tables/English_accents_noise.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{4pt}
\begin{tabular}{ccccccccccccc|c}
\toprule
model & method & f.t. & Al  & Ga & Ha & It & Ku & Li & Me & Ru & Ta & Th  & overall \\
\midrule
conv  & joint  & - & 6.33 & 7.9	& 4.33	& 7.16	& 7.08	& 4.69	& 6.38	& 7.42	& 8.31	& 7.92 & 6.94 \\
conv  & joint  & \checkmark & 6.8 & 6.92 & 5.1 & 7.23 & 7.26 & 5.41 & 8.07 & 7.74 & 8.29 & 7.94 & 7.16 \\
dprnn & joint  & - &7.52 & 9.54	& 6.78 & 8.27 & 8.23 & 5.39	& 8.65	& 8.12	& 8.90	& 8.74 & 8.07\\
dprnn & joint  & \checkmark & 7.93	& 9.17	& 6.6 & 8.14 & 8.06 & 5.89 & 6.68	& 8.19 & 8.66 & 8.86 & 8.06 \\
\midrule
conv  & fomaml & \checkmark & 7.77	& 8.79	& 5.17	& 8.47	& 8.29	& 7.22	& 9.14	& 8.59	& 8.79	& 8.66	& 8.09 \\
conv  & maml   & \checkmark & 7.76 & 9.91 & 5.40 & 9.03 & 8.88	& 7.18 & 8.57 & 9.58 & 10.22 & 9.48 & 8.71 \\
dprnn & fomaml & \checkmark & 8.03	& 9.00	& 7.03	& 8.53	& 8.73	& 6.83	& 9.09	& 8.68	& 8.96	& 8.84	& 8.41\\
\bottomrule
\end{tabular}
\caption{Results of joint training and MAML methods under the 2-speaker setting on the 10 target accents of the Speech Accent Archive. For the Conv-TasNet(conv) and Dual-path RNN(dprnn) model, we mark the highest Si-SNRi values bold.
%For joint training, we report the results with and without fine-tuning.
}
\label{tab:accent_result_2spk}
\end{table*}

==> tables/cv-zh-noise.tex <==
\begin{table}[]
\centering
\setlength\tabcolsep{1.5pt}
\begin{tabular}{ccc|ccc|ccc}
\toprule
      &        &      & \multicolumn{3}{c|}{2-speaker}  & \multicolumn{3}{c}{3-speaker}  \\
model & method & f.t. & zhCN & zhHK & zhTW & zhCN & zhHK & zhTW \\
\midrule
conv  & joint  & -    & 4.36	& 5.38     & 4.16      & 3.27 & 4.83  & 3.05     \\
conv   & joint  & \checkmark    & 4.60   & 5.40   & 4.18     & 3.43 & 4.75   & 3.15     \\
dprnn & joint  & -    & 5.24 & 5.91     & 4.72     & 3.90 & 5.67     & 4.10     \\
dprnn & joint  & \checkmark    & 5.22 & 5.62  &4.53      & 4.00   & 5.73     &4.11      \\
\midrule
conv  & fomaml & \checkmark    &5.99 & 5.73     & 5.21     & 4.58     & 5.86     & 4.32 \\
conv  & maml & \checkmark    & 6.29    & 6.59    & 5.34     &4.91    & 6.81     & 5.49    \\
dprnn & fomaml & \checkmark    & 6.56   & 6.89     & 6.21      & 5.81    & 6.98  & 5.93    \\
\bottomrule
\end{tabular}
\caption{Results of joint training and MAML methods on the testing split of the three CommonVoice Chinese speech data, zh-CN, zh-HK and zh-TW, with Musan noise added.}
\label{tab:CV_noise_results}
\end{table}

==> tables/native-likeness.tex <==
\begin{table}[]
\centering
\begin{tabular}{cccc}
\toprule
accent   & native-likeness & accent     & native-likeness \\
\midrule
albanian & 3.41            & lithuanian & 2.55            \\
ga       & 2.57            & mende      & 3.13            \\
hausa    & 3.18            & russian    & 2.61            \\
italian  & 2.71            & tamil      & 3.4             \\
kurdish  & 2.11            & thai       & 2.38\\
\bottomrule
\end{tabular}
\caption{Native-likeness ratings for the 10 target accents in the testing data.}
\label{tab:native-likeness}
\end{table}

==> tables/pearson_corr.tex <==
\begin{table}[]
\centering
\begin{tabular}{ccccc}
\toprule
model & method & f.t. & 2-speaker & 3-speaker \\
\midrule
conv  & joint  & - & 0.11     & 0.18     \\
conv  & joint  & \checkmark & -0.37     & -0.38     \\
dprnn & joint  & - & 0.23     & -0.13     \\
dprnn & joint  & \checkmark & -0.37     & -0.5    \\
\midrule
conv  & fomaml & \checkmark & 0.01     & -0.04     \\
conv  & maml   & \checkmark & 0.05     & -0.03     \\
dprnn & fomaml & \checkmark & -0.08     & 0.03     \\
\bottomrule
\end{tabular}
\caption{Pearson correlations of the evaluation results and the native-likeness ratings of the utterances in the Speech Accent Archive.}
\label{tab:pear_corr}
\end{table}

==> tables/time.tex <==

\begin{table}[H]
\centering
\begin{tabular}{cc|cc}
\toprule
                      &        & \multicolumn{2}{c}{time (ms)}                                 \\
           model           &   method     & \multicolumn{1}{c}{2-speaker} & \multicolumn{1}{c}{3-speaker} \\
\midrule
\multirow{2}{*}{conv} & fomaml & 1209.27                  & 1411.97                   \\
                      & maml   & 19021.26                   & 19290.09         \\
\bottomrule
\end{tabular}
\caption{Computational time of a meta batch for the Convolutional TasNet model with MAML and FOMAML. The meta batch size is set to 3 and evaluated with milliseconds.}
\label{tab:time}
\end{table}
